Composite Shape Modeling via Latent Space Factorization

We present a novel neural network architecture, termed Decomposer-Composer, for semantic structure-aware 3D shape modeling. Our method utilizes an auto-encoder-based pipeline, and produces a novel factorized shape embedding space, where the semantic structure of the shape collection translates into a data-dependent sub-space factorization, and where shape composition and decomposition become simple linear operations on the embedding coordinates. We further propose to model shape assembly using an explicit learned part deformation module, which utilizes a 3D spatial transformer network to perform an in-network volumetric grid deformation, and which allows us to train the whole system end-to-end. The resulting network allows us to perform part-level shape manipulation, unattainable by existing approaches. Our extensive ablation study, comparison to baseline methods and qualitative analysis demonstrate the improved performance of the proposed method.

==> sections-final/acknowledgements.tex <==
% !TEX root = ../sfp-arxiv-main.tex

\section*{Acknowledgements}
\label{seq:ack}
L. Guibas acknowledges NSF grant CHS-1528025, a Vannevar Bush Faculty Fellowship, and gifts from the Adobe and Autodesk  Corporations.
A. Dubrovina and M. Shalah acknowledge the support in part by The Eric and Wendy Schmidt Postdoctoral Grant for Women in Mathematical and Computing Sciences. F.Xia acknowledges the support from Stanford Graduate Fellowship.


